Weighting Based Approaches to Borrowing Historical Controls for Indirect comparison for Time-to-Event Data with a Cure Fraction

To use historical controls for indirect comparison with single-arm trials, the population difference between data sources should be adjusted to reduce confounding bias. The adjustment is more difficult for time-to-event data with a cure fraction. We propose different adjustment approaches based on pseudo observations and calibration weighting by entropy balancing. We show a simple way to obtain the pseudo observations for the cure rate and propose a simple weighted estimator based on them. Estimation of the survival function in presence of a cure fraction is also considered. Simulations are conducted to examine the proposed approaches. An application to a breast cancer study is presented.

==> newcom.tex <==
\newcommand{\refb}[1]{(\ref{#1})}
\newcommand{\rb}{\right]}
\newcommand{\lb}{\left[}
\newcommand{\lpp}{\left(}
\newcommand{\rpp}{\right)}
\newcommand{\balpha}{{\mbox {\boldmath$\alpha$}}}
\newcommand{\hbalpha}{{\hat {{\mbox {\boldmath$\alpha$}}}}}
\newcommand{\halpha}{{\hat{\alpha}}}
\newcommand{\bbeta}{{\mbox {\boldmath$\beta$}}}
\newcommand{\hbbeta}{{\hat {\mbox {\boldmath$\beta$}}}}
\newcommand{\bdelta}{{\mbox {\boldmath$\delta$}}}
\newcommand{\bDelta}{{\mbox {\boldmath$\Delta$}}}
\newcommand{\bgamma}{{\mbox {\boldmath$\gamma$}}}
\newcommand{\bGamma}{{\mbox {\boldmath$\Gamma$}}}
\newcommand{\blambda}{{\mbox {\boldmath$\lambda$}}}
\newcommand{\bLambda}{{\mbox {\boldmath$\Lambda$}}}
\newcommand{\bdgm}{{\mbox {\boldmath$\digamma$}}}
\newcommand{\bPsi}{{\mbox {\boldmath$\Psi$}}}
\newcommand{\bpsi}{{\mbox {\boldmath$\psi$}}}
\newcommand{\bchi}{{\mbox {\boldmath$\chi$}}}
\newcommand{\bpi}{{\mbox {\boldmath$\pi$}}}
\newcommand{\bphi}{{\mbox {\boldmath$\phi$}}}
\newcommand{\bPhi}{{\mbox {\boldmath$\Phi$}}}
\newcommand{\btheta}{{\mbox {\boldmath$\theta$}}}
\newcommand{\bTheta}{{\mbox {\boldmath$\Theta$}}}
\newcommand{\btau}{{\mbox {\boldmath$\tau$}}}
\newcommand{\bepsi}{{\mbox {\boldmath$\varepsilon$}}}
\newcommand{\hbepsi}{ {\hat {\mbox {\boldmath$\varepsilon$}}}}
\newcommand{\epsi}{\varepsilon}
\newcommand{\bmu}{{\mbox {\boldmath$\mu$}}}
\newcommand{\bnu}{{\mbox {\boldmath$\nu$}}}
\newcommand{\beeta}{{\mbox {\boldmath$\eta$}}}
\newcommand{\bomega}{{\mbox {\boldmath$\omega$}}}
\newcommand{\bzeta}{{\mbox {\boldmath$\zeta$}}}
\newcommand{\bsigma}{{\mbox {\boldmath$\sigma$}}}
\newcommand{\bSigma}{{\mbox {\boldmath$\Sigma$}}}
\newcommand{\hsi}{{\hat{\sigma}}}
\newcommand{\hSi}{{\hat{\Sigma}}}
\newcommand{\bOmega}{{\mbox {\boldmath$\Omega$}}}
\newcommand{\bxi}{{\mbox {\boldmath$\xi$}}}
\newcommand{\bXi}{{\mbox {\boldmath$\Xi$}}}
\newcommand{\tra}{^{\top}}
\newcommand{\bv}{\mbox {\bf v}}
\newcommand{\bV}{\mbox {\bf V}}
\newcommand{\bX}{\mbox {\bf X}}
\newcommand{\bZ}{\mbox {\bf Z}}
\newcommand{\ba}{\mbox {\bf a}}
\newcommand{\ble}{\mbox {\bf e}}
\newcommand{\ha}{\hat{ a}}
\newcommand{\hba}{\hat{{\mbox {\bf a}}}}
\newcommand{\bc}{\mbox {\bf c}}
\newcommand{\bA}{\mbox {\bf A}}
\newcommand{\bB}{\mbox {\bf B}}
\newcommand{\bC}{\mbox {\bf C}}
\newcommand{\bD}{\mbox {\bf D}}
\newcommand{\bE}{\mbox {\bf E}}
\newcommand{\bF}{\mbox {\bf F}}
\newcommand{\mathF}{\mathcal{F}}
\newcommand{\bG}{\mbox {\bf G}}
\newcommand{\bg}{\mbox {\bf g}}
\newcommand{\bH}{\mbox {\bf H}}
\newcommand{\bI}{\mbox {\bf I}}
\newcommand{\bJ}{\mbox {\bf J}}
\newcommand{\bL}{\mbox {\bf L}}
\newcommand{\bM}{\mbox {\bf M}}
\newcommand{\bN}{\mbox {\bf N}}
\newcommand{\bp}{\mbox {\bf p}}
\newcommand{\bO}{\mbox {\bf O}}
\newcommand{\bP}{\mbox {\bf P}}
\newcommand{\bQ}{\mbox {\bf Q}}
\newcommand{\bK}{\mbox {\bf K}}
\newcommand{\bR}{\mbox {\bf R}}
\newcommand{\bT}{\mbox {\bf T}}
\newcommand{\bU}{\mbox {\bf U}}
\newcommand{\bS}{\mbox {\bf S}}
\newcommand{\bW}{\mbox {\bf W}}
\newcommand{\bY}{\mbox {\bf Y}}
\newcommand{\bb}{\mbox {\bf b}}
\newcommand{\bd}{\mbox {\bf d}}
\newcommand{\be}{\mbox {\bf e}}
\newcommand{\blf}{\mbox {\bf f}}
\newcommand{\bk}{\mbox {\bf k}}
\newcommand{\bh}{\mbox {\bf h}}
\newcommand{\bm}{\mbox {\bf m}}
\newcommand{\bn}{\mbox {\bf n}}
\newcommand{\bq}{\mbox {\bf q}}
\newcommand{\bx}{\mbox {\bf x}}
\newcommand{\bly}{\mbox {\bf y}}
\newcommand{\bz}{\mbox {\bf z}}
\newcommand{\br}{\mbox {\bf r}}
\newcommand{\bs}{\mbox {\bf s}}
\newcommand{\bt}{\mbox {\bf t}}
\newcommand{\bu}{\mbox {\bf u}}
\newcommand{\hbui}{\mbox {\bf \hat{u}_i}}
\newcommand{\hui}{\mbox {\hat{u}_i}}
\newcommand{\bw}{\mbox {\bf w}}
\newcommand{\bone}{\mbox {\bf 1}}
\newcommand{\bzer}{\mbox {\bf 0}}
\newcommand{\diag}{\mbox {diag}}
\newcommand{\var}{\mbox {var}}
\newcommand{\cov}{\mbox {cov}}
\newcommand{\cor}{\mbox {cor}}
\newcommand{\tr}{\mbox {tr}}
\newcommand{\ee}{\mbox {e}}
\newcommand{\lgt}{\mbox {logit}}
\newcommand{\beqn}{\begin {equation}}
\newcommand{\eeqn}{\end {equation}}
\newcommand{\beqa}{\begin {eqnarray}}
\newcommand{\eeqa}{\end {eqnarray}}
\newcommand{\ssqe}{\sigma^2_e}
\newcommand{\ssqu}{\sigma^2_u}
\newcommand{\half} {\frac {1}{2}}
\newcommand{\pqpt} {\partial {\bf q}/\partial {\bf \theta}}
\newcommand{\pqipt} {\partial {\bf q}_i/\partial {\bf \theta}}
\newcommand{\pqpts} {\partial^2 {\bf q}_i/\partial {\bf \theta} \partial {\bf \btheta^\top}}
\newcommand{\pfpt} {\partial {\bf h}/\partial {\bf \theta}}
\newcommand{\pfipt} {\partial {\bf h}_i/\partial {\bf \theta}}
\newcommand{\pfpts} {\partial^2 {\bf h}/\partial {\bf \theta} \partial {\bf \theta^\top}}
\newcommand{\pfipts}{\partial^2 {\bf h}_i/\partial {\bf \theta} \partial {\bf \theta^\top}}
\newcommand{\pfopts}{\partial^2 {\bf h}_1/\partial {\bf \theta} \partial {\bf \theta^\top}}
\newcommand{\pfmpts}{\partial^2 {\bf h}_m/\partial {\bf \theta} \partial {\bf \theta^\top}}
\newcommand{\pqipts}{\partial^2 {\bf q}_i/\partial {\bf \theta} \partial {\bf \theta^\top}}
\newcommand{\phpt}{\frac{\partial h}{\partial \btheta}}
\newcommand{\ft}{{\bf f(\theta,X_i)}}
\newcommand{\ftu}{{\bf f(\theta+u,X)}}
\newcommand{\fu} {{\bf f(\theta,X)}}
\newcommand{\sumi} {\sum_{i=1}^m}
\newcommand{\sumni} {\sum_{j=1}^{n_i}}
\newcommand{\ind} {\perp \!\!\!\perp}
\newcommand{\sigse} {\sigma_e^2}
\newcommand{\sigsu} {\sigma_u^2}
\newcommand{\sigu} {\sigma_u^2}
\newcommand{\pp}[2]{\frac{\partial #1}{\partial #2}}
\newcommand{\ppt}[2]{\frac{\partial^2 #1}{\partial #2 \partial {#2}^\top}}
\newcommand{\ppp}[3]{\frac{\partial^2 #1}{\partial #2 \partial #3}}
\newcommand{\ppl}[2]{\partial #1 / \partial #2}
\newcommand{\pppl}[3]{\partial^2 #1 / \partial #2 \partial #3 }
\newcommand{\bvbt}{\begin{verbatim}}
\newcommand{\benu}{\begin{enumerate}}
\newcommand{\eenu}{\end{enumerate}}
\newcommand{\bver}{\begin{verbatim}}
\def\beq{&~=~&}
\newcommand{\hbe}{\bar{\be}}
\newcommand{\nn}{\nonumber}
\makeatletter
\input{rotate}\newbox\rotbox
\newenvironment{sidetable}{\begin{table}[t]
\global\setbox\rotbox\vbox\bgroup
\hsize\textheight \@parboxrestore}%
{\par\vskip\z@\egroup \rotl\rotbox \end{table}}
\makeatother
\newdimen\x \x=1.5mm











